Strategyproof Decision-Making in Panel Data Settings and Beyond

We consider the problem of decision-making using panel data, in which a decision-maker gets noisy, repeated measurements of multiple units (or agents). We consider a setup where there is a pre-intervention period, when the principal observes the outcomes of each unit, after which the principal uses these observations to assign a treatment to each unit. Unlike this classical setting, we permit the units generating the panel data to be strategic, i.e. units may modify their pre-intervention outcomes in order to receive a more desirable intervention. The principal's goal is to design a strategyproof intervention policy, i.e. a policy that assigns units to their utility-maximizing interventions despite their potential strategizing. We first identify a necessary and sufficient condition under which a strategyproof intervention policy exists, and provide a strategyproof mechanism with a simple closed form when one does exist. Along the way, we prove impossibility results for strategic multiclass classification, which may be of independent interest. When there are two interventions, we establish that there always exists a strategyproof mechanism, and provide an algorithm for learning such a mechanism. For three or more interventions, we provide an algorithm for learning a strategyproof mechanism if there exists a sufficiently large gap in the principal's rewards between different interventions. Finally, we empirically evaluate our model using real-world panel data collected from product sales over 18 months. We find that our methods compare favorably to baselines which do not take strategic interactions into consideration, even in the presence of model misspecification.

==> content/existence-old.tex <==
%\section{Intervening Under Strategic Responses}


\section{Characterizing Strategyproof Intervention Policies}\label{sec:characterizing}
To define the condition under which a strategyproof intervention policy exists, we need to first introduce the notion of a \emph{best-response ball}.
\begin{definition}[Best-Response Ball]\label{def:ball}
    The best-response ball of a set of units $\cV$ is the set of all pre-intervention outcomes $\cB(\cV)$ such that
    \begin{equation*}
        \Tilde{\vy}_{pre} \in \cB(\cV) \; \text{ if } \; \left\| \Tilde{\vy}_{pre} - \vy_{v, pre} \right\|_2 \leq \delta \text{ for any } v \in \cV,
    \end{equation*}
    where $\vy_{pre,v} \in \cY_{pre}$ denotes the pre-intervention outcomes associated with unit $v$. We say that $\Tilde{\vy}_{pre}$ is reachable by some unit in $\cV$ if $\Tilde{\vy}_{pre} \in \cB(\cV)$.
\end{definition}
The best-response ball for a unit is its set of feasible manipulations according to~\Cref{ass:mod}. The best-response ball for a set of units is simply the union of the balls of all units contained within the set. Equipped with this definition, we are now ready to introduce the sufficient and necessary condition for a strategyproof intervention policy to exist.

\begin{condition}\label{cond:nec-suf}
For all interventions $d \in \range{k}_0$, there does not exist any unit $v$ belonging to $\pv{\cV}{d}$ whose best-response ball $\cB(v)$ is a complete subset of the best-response balls of units with types less than $d$. Formally,
\begin{equation*}
    \forall d \in \range{k}_0, \; \not \exists \; v \in \pv{\cV}{d} \text{ s.t. } \cB(v) \subseteq \bigcup_{d' = 0}^{d-1} \cB(\pv{\cV}{d'}).
\end{equation*}
\end{condition}

\begin{theorem}\label{thm:impossible}
    Under the setting of~\Cref{sec:setting},~\Cref{cond:nec-suf} is both necessary and sufficient for a strategyproof intervention policy (as defined in~\Cref{def:spip}) to exist.
\end{theorem}
\noindent The following two lemmas (\Cref{lem:nec} and~\Cref{lem:suf}) immediately imply~\Cref{thm:impossible}.
\begin{lemma}\label{lem:nec}
    Suppose \Cref{cond:nec-suf} does not hold. Then there exists no mapping $\pi: \mathcal{Y}_{pre} \rightarrow \range{k}_0$ which can intervene perfectly on all units types.
\end{lemma}
\begin{proof}
    Let~\Cref{cond:nec-suf} be violated for some unit $v \in \pv{\cV}{d}$. Since $$\cB(v) \subseteq \bigcup_{d' = 0}^{d-1} \cB(\pv{\cV}{d'}),$$ any valid modified pre-treatment behavior of unit $v$ can also be obtained by some other unit $v' \in \bigcup_{d' = 0}^{d-1} \pv{\cV}{d'}$ by~\Cref{def:ball}.
    Therefore, no intervention policy can perfectly intervene on both $\pv{\cV}{d}$ and $\{\pv{\cV}{d'}\}_{d'=1}^{d-1}$.
\end{proof}
\iffalse
{\color{blue} Is there a ``localized'' version of this statement? So we can verify it for every intervention $d \in [k]_0$ separately? That is, we can have strategyproofness for a subset of the interventions / units.}

{\color{blue} Does this implicitly assume that the points where $[\mathcal{V}^{d'}]_{d' \in [d - 1]}$ are incentivized to move to, the units in $\mathcal{V}^{d}$ are not incentized to move to?}
\fi 
\begin{algorithm}[t]
        \SetAlgoNoLine
        Let $\mathcal{S} = \cB \left( \bigcup_{d=0}^{d=k-1} \pv{\cV}{d} \right)$\\
        \For{$d = (k-1), \ldots, 1$}
        {
            Let 
            \begin{equation*}
                \pv{\mathcal{Y}}{d}_{pre} = \left( \cB(\pv{\cV}{d}) /\ \bigcup_{d' = 0}^{d-1} \cB(\pv{\cV}{d'}) \right) \cap \mathcal{S}
            \end{equation*}
            $\mathcal{S} = \mathcal{S} /\ \pv{\mathcal{Y}}{d}_{pre}$
        }
        Let $\pv{\mathcal{Y}}{0}_{pre} = \mathcal{S}$\\
        For $\Tilde{\vy}_{pre} \in \cB \left( \bigcup_{d=0}^{d=k-1} \pv{\cV}{d} \right)$, assign the intervention $d$ s.t. $\Tilde{\vy}_{pre} \in \pv{\cY}{d}_{pre}$.
        \caption{Strategyproof Interventions on Panel Data}
        \label{alg:sp-multi-opt}
\end{algorithm}

Next we show that~\Cref{cond:nec-suf} is sufficient for a strategyproof intervention policy to exist, by providing an algorithm (\Cref{alg:sp-multi-opt}) for constructing a strategyproof intervention policy whenever~\Cref{cond:nec-suf} holds.~\Cref{alg:sp-multi-opt} proceeds by partitioning the set of all reachable pre-treatment outcomes (denoted by $\cB \left( \bigcup_{d=0}^{d=k-1} \pv{\cV}{d} \right)$) into sets $\{ \pv{\cY}{d}_{pre}\}_{d=0}^{k-1}$ in order of decreasing unit intervention preference. Each partition $\pv{\cY}{d}_{pre}$ is 
the subset of $\cY_{pre}$ that is (1) only reachable 
by units of type
$d' \geq d$ and (2) reachable by every unit of type $d$. Finally,~\Cref{alg:sp-multi-opt} assigns intervention $d$ to a unit $v$ only if $\Tilde{\vy}_{v,pre} \in \pv{\cY}{d}_{pre}$, where $\Tilde{\vy}_{v,pre}$ denotes unit $v$'s modified pre-treatment outcomes.

\begin{lemma}\label{lem:suf}
    Suppose~\Cref{cond:nec-suf} holds. Then~\Cref{alg:sp-multi-opt} gives a strategyproof intervention policy according to~\Cref{def:spip}.
\end{lemma}
\begin{proof}
Consider the intervention policy in~\Cref{alg:sp-multi-opt}.
By construction, no units with type $d' < d$ can modify their pre-intervention outcomes to receive intervention $d$. Since~\Cref{cond:nec-suf} holds, by~\Cref{ass:mod} all units of type $d$ will have at least one feasible set of modified pre-treatment outcomes $\Tilde{\vy}_{pre}$ such that $\Tilde{\vy}_{pre} \in \pv{\cY}{d}_{pre}.$
Finally, note that units with type $d' > d$ have no incentive to receive intervention $d$.
\end{proof}
While the construction of~\Cref{alg:sp-multi-opt} is
proof of the existence of a strategyproof intervention policy,
there is no guarantee that $\pv{\cY}{d}_{pre}$ can be computed in an efficient manner for arbitrary distributions over unit types. In the sequel, we specialize our results to the case where outcomes are generated via a latent factor model, and show that under this setting, the strategyproof intervention policy of~\Cref{alg:sp-multi-opt} takes a simple closed form.\looseness-1

==> content/intro.tex <==
\section{Introduction}
%
In panel data settings (also known as longitudinal data settings) one observes repeated, noisy, measurements of a collection of  \emph{units} over a period of time, undergoing different interventions.
%
Units can range from individuals, companies, or even geographic locations; interventions can range from discounts, health therapies, or, say, tax regulations.
%
This is a ubiquitous way to collect data, and, as a result, the analysis of panel data has a long history in econometrics and statistics.
%
A common goal in the literature is to analyze how a \emph{principal} (e.g., business platform, regulatory agency) can do ``counterfactual inference'', i.e., estimate what will happen to a unit if it undergoes a variety of possible interventions.
%
The ultimate goal of such counterfactual inference is to enable data-driven decision-making, where one does not just estimate statistical parameters of interest, but actually uses data to make better decisions. In medical domains, for example, the goal typically is not just estimating  health outcomes for patients under different health therapies, but also a policy that selects appropriate therapies for new patients.
%
However, the leap from counterfactual inference to data-driven decision-making comes with additional challenges: namely, units have incentives to behave strategically when they have much to gain or lose from the intervention they are assigned.\looseness-1

%
A running example we will use throughout this paper is that of an e-commerce platform that wishes to give one of several possible discounts to a new user to maximize some future metric of interest, say, engagement levels. 
%
Suppose the company uses historical data to build a model that estimates the ``counterfactual'' trajectory of engagement levels of a new user under different discount policies, based on their observed trajectory of engagement levels thus far.
%
If a user knew this were the case, then there is a clear incentive for them to strategically modify their engagement levels to receive a larger discount.
%
Such strategic manipulations in response to data-driven decision-making have also been observed in other domains such as lending \citep{homonoff2021does} and search engine optimization \citep{davis2006search}.
%
%Hence, we focus on two natural questions that arise as we transition from counterfactual inference to decision-making: 
In this paper, we focus on \emph{strategyproof} intervention policies, i.e., policies that assign the correct treatment to the units despite them strategically altering their data. Concretely, we answer two questions:

\vspace{-3mm}

{\centerline \em {\bf Q1:} Is it possible to design strategyproof estimators that are robust to strategic modification of data by units to receive a more favorable intervention?}

\vspace{-3mm}

{\centerline \em {\bf Q2:} Can we leverage the structure typically present in panel data to derive computationally-efficient algorithms for learning strategyproof estimators?}

%\vspace{2mm}
%
Towards answering both questions, and in line with the e-commerce example described above, we build upon the framework for counterfactual inference with panel data called \emph{synthetic interventions} \citep{SI}, which itself is a generalization of the canonical framework called \emph{synthetic controls} \citep{abadie2003economic, abadie2010synthetic}.
%
In both settings, there is a notion of a ``pre-intervention'' period when all units are under control (i.e., no intervention), and then a ``post-intervention'' period, when each unit undergoes \emph{exactly one} of many possible interventions (including control).
%
Synthetic controls can be used to estimate the counterfactual outcome if a unit did not undergo an intervention, i.e., remained under control.
%
Given its simplicity, synthetic controls has become a ubiquitous technique in econometrics to estimate counterfactuals under control in high-stakes domains including e-commerce, healthcare, and policy evaluation. 
%
Synthetic interventions is a generalization which allows one to estimate counterfactual outcomes not just under control, but also under intervention.
%
Despite being a relatively new development, the synthetic interventions framework has been used by several companies across therapeutics, ride-sharing, and e-commerce, to estimate the best intervention for a given unit. 
%

Given the growing popularity of the synthetic interventions (and synthetic controls) framework in high-stakes decision-making, an issue that will likely arise is the strategic manipulation of observed outcomes by units. 
%
In particular, just as in the e-commerce example, units have an incentive to manipulate their pre-intervention outcomes to get a more favorable intervention during the post-intervention period. 
%
Indeed, if such strategic manipulations are not taken into account, we establish that the synthetic interventions estimator can perform poorly---see~\Cref{sec:not-sp} for a formal example of such a scenario and~\Cref{sec:experiments} for an empirical example based on real-world e-commerce data.\looseness-1

%
The goal of the principal in such settings is to assign the ``correct'' intervention to each unit---the intervention which maximizes some objective function such as total user engagement---during the post-intervention period, despite possible strategic manipulations to the unit's pre-treatment behavior. 
%
As we observe, this can be thought of as designing a mechanism for {\em strategyproof multi-class classification} with panel data.
%
Although many of our results apply more broadly to strategyproof multi-class classification, we focus on panel data (and in particular the setup of synthetic interventions and synthetic controls) due to its ubiquity and for concreteness.

%further, we find that a latent factor model assumption typically made in panel data settings leads to surprisingly simple closed-form strategyproof estimators.  

\subsection{Our contributions}


\iffalse
Our main contribution is to develop a general framework for decision-making in the presence of strategic agents in the panel data setting.
%
See~\Cref{fig:summary} for a summary of our framework. 
%
Under this setting, we provide a necessary and sufficient condition for a strategyproof mechanism for assigning interventions in the post-intervention period to exist, and characterize the optimal mechanism when one does exist. 
%
Next, we specialize our results to the setting in which unit outcomes are determined via a latent factor model, a standard assumption in the panel data setting. 
%
We show that under a latent factor model and a linearity assumption on principal reward, a strategyproof mechanism takes a simple closed form when one exists. 
%
Additionally, we show that a strategyproof mechanism always exists when there is only a single treatment and control---this is generally not the case when there is more than one treatment.
%
Our results imply an impossibility result for multi-class classification under incentives, which may be of independent interest; namely, there exist settings in which perfect multi-class classification is not possible when making decisions about agents with incentive to behave strategically, {\em even} if the initial agent population is linearly separable.
%
Next, we provide an algorithm for learning a strategyproof mechanism when the principal has access to historical data, and provide performance guarantees in the setting where there is a single treatment. 
%
When there are multiple treatments, we show that similar finite sample guarantees hold if there exists a sufficiently large gap in rewards between the different interventions.
%
Finally, we empirically evaluate the effects of model misspecification on principal utility using semi-synthetic data constructed from product sales over the course of 18 months.
\looseness-1
\fi 

The first contribution of our work is a general framework for decision-making in the presence of strategic agents in the panel data setting. 
%
Our model is formally defined in Section~\ref{sec:setting}, but for the purposes of exposition, we outline it informally here as well. 
%
In our setting, a principal originally observes historical data from pre- and post- intervention outcomes of $n$ units. 
%
Each of these units $i \in \{1, \ldots, n\}$ is randomly assigned an intervention $d_i$ as in an A/B test (i.e., a randomized control trial), so they do not have incentive to strategize with their pre-intervention outcomes. 
%
After observing this historical data, the principal commits to an intervention policy $\pi$, which uses a unit's pre-intervention outcomes to assign its intervention during the post-intervention period. 
%
Then $m$ new units arrive and potentially strategically modify their pre-treatment outcomes; units are allowed to move in a ball of radius $\delta$ around their true pre-intervention outcomes, but they are not further constrained. 
%
We call this behavior \emph{best-responding} and formally define it in Definition~\ref{ass:mod}. 
%
Finally, the principal observes the altered pre-intervention outcomes, assigns interventions according to policy $\pi$, and collects the post-intervention rewards. 
%
Figure~\ref{fig:summary} presents a summary of our framework. The goal of the principal in this setting is to deploy a policy $\pi$ that is \emph{strategyproof}, i.e., assigns the ``correct'' intervention to all units, despite the fact that they may have strategically modified their pre-intervention outcomes. 
%
We call this ``correct'' intervention the unit's \emph{type}.
\begin{figure}[htbp]
    \centering
    \noindent \fbox{\parbox{0.95\textwidth}{
    \vspace{0.1cm}
    \textbf{Protocol: Decision-Making in the Presence of Strategic Units in the Panel Data Setting}
    
    \vspace{-0.2cm}
    %\noindent\rule{15.9cm}{0.4pt}
    %\noindent\rule{15.1cm}{0.4pt}
    \noindent\rule{13.2cm}{0.4pt}\vspace{1mm}
    \begin{enumerate}
        %\setcounter{enumi}{-1}
        \item Principal observes historical data $\{(\vy_{i,pre}, \vy_{i,post}^{(d_i)})\}_{i=1}^n$\vspace{2mm}
        %
        \item Principal commits to an intervention policy $\pi: \mathcal{Y}_{pre} \rightarrow \{0, \ldots, k-1\}$\vspace{2mm}
        %
        \item $m$ new units arrive and strategically modify their pre-treatment outcomes from $\{\vy_{i, pre}\}_{i=n+1}^{n+m}$ to $\{\Tilde{\vy}_{i, pre}\}_{i=n+1}^{n+m}$ according to~\Cref{ass:mod}.\vspace{2mm} 
        %
        \item Principal observes $\{\Tilde{\vy}_{i, pre}\}_{i=n+1}^{n+m}$ and assigns interventions $\{d_{i}^{\pi} := \pi(\Tilde{\vy}_{i, pre})\}_{i=n+1}^{n+m}$\vspace{2mm}
        %
        \item Principal receives rewards $\{\pv{r}{d_{i}^{\pi}}_{i} = f(\pv{\vy}{d_i^{\pi}}_{i,post})\}_{i=n+1}^{n+m}$\vspace{1mm}
        %
    \end{enumerate}
    }}
    \caption{Protocol for decision-making in panel data settings under strategic responses.}
    \label{fig:summary}
\end{figure}


Given that units know the principal's policy $\pi$ and they are allowed to best respond anywhere within $\delta$ of their true pre-intervention outcome, it may seem like {\bf Q1} has a negative answer. However, in Section~\ref{sec:characterizing}, we derive the \emph{necessary and sufficient conditions} for a strategyproof intervention policy to exist. On a technical level, in order to obtain this full characterization, we translate our problem to the dual space (i.e., the space of the units' actions), and derive properties that units of the same type must share. Intuitively, our necessary condition (\Cref{lem:nec}) says that the units must be adequately different in terms of their true types. Our sufficient condition (\Cref{lem:suf}) presents a specific policy which optimally assigns units to interventions by incentivizing some units to strategize.\looseness-1

Our next contribution is to specialize our characterization of strategyproof intervention policies to the setting where unit outcomes at each round are determined by a latent factor model. 
%
Under a latent factor model (a natural and popular assumption in panel data settings), unit outcomes under different interventions are linearly dependent on a unit latent factor (i.e, their type), as well as a latent vector that is time- and intervention-specific. 
%
In this specification, the rewards of the principal also follow a linear structure, which implies the units are {\em linearly separable} based on their type.
%
We show that our necessary and sufficient condition for a strategyproof intervention policy to exist is satisfied when there are two interventions (\Cref{cor:two}), but it is in general \emph{not} satisfied for more than two (\Cref{ex:impossible}). 
%
The intuition for both results is that in order for an intervention policy to be strategyproof under the latent factor model, the principal has to shift the decision boundaries by some amount in order to account for the fact that units are able to strategize. 
%
When the number of interventions is more than two, it may be the case that there are units of different types whose pre-intervention outcomes are close enough to each other such that no movement of the boundary can stop all units from fooling the principal. 
%
Importantly, in Section~\ref{sec:lfm} we show that assigning three or more interventions in a panel data setting with strategic agents can be interpreted as an instance of \emph{multi-class strategic classification}. 
%
As such, our impossibility result for strategyproof intervention policies translates to an impossibility result for strategyproof classification with three or more classes. 
%
To the best of our knowledge, we are the first to both draw this connection, and discuss multi-class strategic classification altogether. 

Having characterized strategyproof intervention policies under a latent factor model, we shift our focus to {\bf Q2}. For the case where there is a single treatment and control, we provide an algorithm for learning a strategyproof intervention policy from historical data (\Cref{alg:sp-two-action}). 
%
The analysis of~\Cref{alg:sp-two-action} relies on two steps: First, we upper-bound the difference between the reward of the learned policy and that of the optimal policy by the estimation error of the relationship between pre-intervention outcomes and rewards on the historical data (\Cref{cor:two-learn}). 
%
Second, we leverage bounds for estimation from the ``error-in-variables'' literature to derive end-to-end finite sample guarantees (\Cref{thm:out-of-sample-informal}). 
%
We show that under relatively minor algebraic assumptions, our intervention policy is asymptotically optimal in the limit of infinite data. 
%
Next, we provide analogous finite sample guarantees for an extension of~\Cref{alg:sp-two-action} to the setting with an arbitrary number of treatments (\Cref{alg:learning-sp})---under an additional assumption on the difference in rewards between the optimal and next-best intervention for each type of unit (\Cref{thm:main}). 
%
Relaxing this assumption on the reward gap appears challenging; we provide evidence for the necessity of such a condition in~\Cref{ex:1D}.

%
Finally, we complement our theoretical results with experiments based on panel data from product sales at several stores over the course of 18 months. 
%
We find the data is well-approximated by a latent factor model, and that the intervention policy of~\Cref{alg:sp-two-action} outperforms a baseline policy which does not take strategic interactions into consideration---even when the algorithm's estimate of $\delta$ (the unit effort budget) is misspecified. 

==> content/lfm-old.tex <==
\section{Strategyproof Interventions Under Latent Factor Models}\label{sec:lfm}
We now specialize our results to the setting in which unit outcomes at each time-step are determined by a \emph{latent factor model}, a popular assumption in the panel data setting (see, e.g., the references in~\Cref{sec:related}).

\begin{assumption}[Latent Factor Model]\label{ass:lfm}
Suppose the outcome for unit $i$ at time $t$ under treatment $d \in \range{k}_0$ takes the following factorized form
\begin{equation}\label{eq:lfm}
\begin{aligned}
    y_{i,t}^{(d)} &= \langle \vu_t^{(d)}, \mathbf{v}_i \rangle\\
    \pv{\mathring{y}}{d}_{i,t} &= y_{i,t}^{(d)} + \varepsilon_{i,t}
\end{aligned}
\end{equation}
where $\vu_t^{(d)} \in \mathbb{R}^r$ is a latent vector which depends only on the time-step $t$ and intervention $d$, $\mathbf{v}_i \in \mathbb{R}^r$ is a latent vector which only depends on unit $i$ (i.e., unit $i$'s \emph{private type}), and $\varepsilon_{i,t}^{(d)}$ is zero-mean sub-Gaussian random noise with variance  $\sigma^2$. For simplicity, we assume that $|\pv{y}{d}_{i,t}| \leq 1, \; \forall \; i \in \range{m}, t \in \range{T}, d \in \range{k}_0$.
\end{assumption}
Note that under~\Cref{ass:lfm}, the principal does not need to know $\vu_t^{(d)}$ or $\mathbf{v}_i$.
We assume that $r$ is known to the principal for ease of analysis, although several principled heuristics exist for estimating $r$ in practice from data. See, e.g., \citet[Section 2.2.1]{SI} for details. Additionally, we impose the following linearity assumption on the principal's reward function:\looseness-1

\begin{assumption}(Linearity of Rewards)\label{ass:reward}
We assume that the principal's reward for unit $i$ under intervention $d$ is a weighted sum of unit $i$'s outcomes in the post-treatment time period. Specifically,
\begin{equation}\label{eqn:reward}
    r_i^{(d)} = \sum_{t = T_0 + 1}^N \omega_t \cdot y_{i,t}^{(d)},
\end{equation}
where $\omega_t \in \mathbb{R}$ for $t > T_0$.
\end{assumption}

This corresponds to the setting in which the principal wants to assign an intervention to \emph{maximize} some linear combination of each unit's post-intervention outcomes. Such an assumption is often reasonable under many settings; for example, in e-commerce, the online marketplace may wish to maximize the total amount of user engagement on the platform in the post-intervention period (this corresponds to the setting in which $\omega_{t} = 1$ for $t > T_0$).

Next we show that under~\Cref{ass:lfm} and~\Cref{ass:reward},
the principal's reward can be rewritten as a function of their pre-treatment outcomes.
Note that by~\Cref{ass:lfm}, $\vy_{i,pre}$ has the following equivalent matrix-vector factorization:
\begin{equation}\label{eqn:mat-vec}
    \vy_{i,pre} = U \mathbf{v}_i,
\end{equation}
where $U \in \mathbb{R}^{T_0 \times r}$ is the matrix with rows $\vu_1^{(0)\top}, \ldots, \vu_{T_0}^{(0)\top}$.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\textwidth]{figure/two-interventions.png}
    \caption{(Left:~\Cref{prop:reward}) The optimal policy in the non-strategic setting assigns the control (intervention $0$) to the units left of the line $\langle \pv{\vbeta}{1} - \pv{\vbeta}{0}, \vy_{pre} \rangle = 0$ (in blue) and intervention $1$ to the units to the right. (Right:~\Cref{cor:simplified}) When units are strategic, the optimal decision boundary is shifted by $\delta$ in the direction of $\pv{\vbeta}{1} - \pv{\vbeta}{0}$.}
    \label{fig:two-intervention-visual}
\end{figure}

\begin{proposition}[Principal Reward Reformulation]\label{prop:reward}
    If $U$ has full column rank, $r_i^{(d)}$ can be rewritten as
    \begin{equation*}
        r_i^{(d)} = \langle \pv{\vbeta}{d}, \vy_{i,pre} \rangle,
    \end{equation*}
    where $$\pv{\vbeta}{d} := U (U^\top U)^{-1} \sum_{t = T_0 + 1}^T \omega_t \cdot \vu_t^{(d)}.$$
\end{proposition}
\begin{proof}
    Rearranging~\Cref{eqn:mat-vec}, we see that 
    \begin{equation*}
    \begin{aligned}
        \mathbf{v}_i &= (U^\top U)^{-1} U^\top \vy_{i,pre}.
    \end{aligned}
    \end{equation*}
    Using~\Cref{eq:lfm} and substituting the expression for $\mathbf{v}_i$ into~\Cref{eqn:reward}, we see that
    \begin{equation*}
    \begin{aligned}
        r_i^{(d)} &= \sum_{t = T_0 + 1}^T \omega_t \cdot \langle \vu_t^{(d)}, \mathbf{v}_i \rangle\\
        &= \left \langle \sum_{t = T_0 + 1}^T \omega_t \cdot \vu_t^{(d)}, (U^\top U)^{-1} U^\top \vy_{i,pre} \right \rangle.
    \end{aligned}
    \end{equation*}
    Rearranging terms obtains the result.
\end{proof}

The assumption of full column rank on $U$ is relatively minor as long as $T_0 > r$. Such an assumption is commonplace under latent factor models, where the dimension of the latent factors $r$ is usually assumed to be small relative to the other parameters of the problem. Using this reward reformulation, we are able to show that the intervention policy of~\Cref{alg:sp-multi-opt} takes a relatively simple closed-form expression.

\begin{corollary}\label{cor:simplified}
    Under~\Cref{ass:lfm}, and~\Cref{ass:reward}, the following intervention policy is strategyproof as long as~\Cref{cond:nec-suf} holds:

    Assign intervention $d$ if
    \begin{equation}\label{eqn:opt-ip}
    \begin{aligned}
        \langle \pv{\vbeta}{d} - \pv{\vbeta}{d'}, \Tilde{\vy}_{pre} \rangle - \delta \| \pv{\vbeta}{d} - \pv{\vbeta}{d'} \|_2 &> 0 \; \text{ for all } \; d' < d\\
        \text{and } \; \langle \pv{\vbeta}{d} - \pv{\vbeta}{d'}, \Tilde{\vy}_{pre} \rangle + \delta \| \pv{\vbeta}{d} - \pv{\vbeta}{d'} \|_2 &\geq 0 \; \text{ for all } \; d' > d.
    \end{aligned}
    \end{equation}
\end{corollary}
\begin{proof}
    The proof follows by applying the reward reformulation of~\Cref{prop:reward} (which holds under Assumptions \ref{ass:lfm} and \ref{ass:reward}) to~\Cref{alg:sp-multi-opt}.
    Observe that by using~\Cref{prop:reward}, $\cB(\pv{\cV}{d})$ may be defined as
    \begin{equation*}
    \begin{aligned}
        \Tilde{\vy}_{pre} \in \cB(\pv{\cV}{d}) \; \text{ if } \; &\| \Tilde{\vy}_{pre} - \vy_{v,pre} \|_2 \leq \delta,\\
        \text{for any } \; \vy_{v,pre} \; \text{ such that } \; &\langle \pv{\vbeta}{d} - \pv{\vbeta}{d'}, \vy_{v,pre} \rangle \geq 0 \; \text{ for all } \; d' \in \range{k}_0.
    \end{aligned}
    \end{equation*}
    Equivalently,
    \begin{equation*}
    \begin{aligned}
        \Tilde{\vy}_{pre} \in \cB(\pv{\cV}{d}) \; \text{ if } \; &\langle \pv{\vbeta}{d} - \pv{\vbeta}{d'}, \Tilde{\vy}_{pre} \rangle + \delta \| \pv{\vbeta}{d} - \pv{\vbeta}{d'} \|_2 \geq 0 \; \text{ for all } \; d' \in \range{k}_0.
    \end{aligned}
    \end{equation*}
    Applying the definition of $\pv{\cY}{d}_{pre}$ from~\Cref{alg:sp-multi-opt} obtains the result.
\end{proof}
Intuitively, the intervention policy of~\Cref{cor:simplified} can be thought of as computing $\pv{\cY}{d}_{pre}$ by first starting with the set of all $\vy_{pre}$ corresponding to units with type $d$ under no modification, and appropriately shifting the boundaries to account for strategic manipulations. By ``shrinking'' the regions corresponding to interventions which are more desirable to units, the principal is able to disincentivize units from manipulating in order to receive an intervention $d'$ other than their type $d$. Since~\Cref{cond:nec-suf} holds, all units with type $d$ will be able to appropriately modify their pre-treatment outcomes in order to receive intervention $d$. See~\Cref{fig:two-intervention-visual} for an illustration of the intervention policy of~\Cref{cor:simplified} when $d \in \{0, 1\}$. Next we show that under~\Cref{ass:lfm} and~\Cref{ass:reward},~\Cref{cond:nec-suf} always holds for the special case where $d \in \{0, 1\}$, i.e., when there is only one treatment and control.

\begin{corollary}\label{cor:two}
    If $d \in \{0, 1\}$,~\Cref{cond:nec-suf} always holds under~\Cref{ass:lfm} and~\Cref{ass:reward}.\looseness-1
\end{corollary}
\begin{proof}
    If $d \in \{0, 1\}$,~\Cref{cond:nec-suf} simplifies to 
    \begin{equation*}
        \not \exists \; v \in \pv{\cV}{1} \text{ s.t. } \cB(v) \subseteq \cB(\pv{\cV}{0}).
    \end{equation*}
    By~\Cref{prop:reward}, $\pv{\cV}{0}$ and $\pv{\cV}{1}$ are separated by a single hyperplane. Therefore by~\Cref{def:ball}, the simplified version of~\Cref{cond:nec-suf} must hold.
\end{proof}
\Cref{cond:nec-suf} is always satisfied when $d \in \{0, 1\}$ since the latent factor model and linear principal reward imply that there is a single hyperplane separating $\pv{\cV}{0}$ and $\pv{\cV}{1}$. Therefore, if a unit of type $1$ modifies in the direction of this hyperplane by $\delta$, they are guaranteed to receive treatment.
Note that this is generally not the case when the number of interventions $k \geq 3$. To see this, consider the following example:
\begin{example}\label{ex:impossible}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.38\textwidth]{figure/bad-example.png}
    \caption{Visualization of the space of pre-intervention outcomes from~\Cref{ex:impossible}. Blue lines represent optimal decision boundaries in the non-strategic setting. One distribution over unit types for which perfect decision making is not possible in the strategic setting puts non-zero probability on the orange dot ($\pv{\mathbf{v}}{2}$) and both of the orange lines (left: $\pv{\cV}{0}$, right: $\pv{\cV}{1}$). (Recall that in this example, $\pv{u}{0}_1, \pv{u}{0}_2$ are such that $\vy_{\mathbf{v},pre} = \mathbf{v}$.)}
    \label{fig:bad-example}
\end{figure}
Suppose $d \in \{0, 1, 2\}$, $T_0 = 2$, and units prefer intervention $2$ over interventions $1$ and $0$, of which they are indifferent between. Suppose that
\begin{itemize}
    \item $\pv{\vbeta}{0} = [-1 \;\; 0.5]^\top$,
    \item $\pv{\vbeta}{1} = [1 \;\; 0.5]^\top$,
    \item $\pv{\vbeta}{2} = [0 \;\; 1]^\top$, and
    \item $\vy_{\mathbf{v},pre} = \mathbf{v}$.\footnote{Such a setting is possible, e.g., when $\pv{\vu}{0}_1 = [1 \;\; 0]^\top$, $\pv{\vu}{0}_2 = [0 \;\; 1]^\top$, $\sum_{t=T_0+1}^T \pv{\vu}{0}_t = [-1 \;\; 0.5]^\top$, $\sum_{t=T_0+1}^T \pv{\vu}{1}_t = [1 \;\; 0.5]^\top$, $\sum_{t=T_0+1}^T \pv{\vu}{2}_t = [0 \;\; 1]^\top$, and $\omega_{T_0 + 1} = \omega_{T_0 + 2} = \cdots = \omega_{T} = 1$.}
\end{itemize}

Consider the following set of unit types: Let
\begin{itemize}
    \item $\pv{\mathcal{V}}{0} = \{\mathbf{v} \; : \; \langle \pv{\vbeta}{2} - \pv{\vbeta}{0}, \mathbf{v} \rangle = -\alpha, \; \mathbf{v}[1] < 0 \}$, 
    \item $\pv{\mathcal{V}}{1} = \{\mathbf{v} \; : \; \langle \pv{\vbeta}{2} - \pv{\vbeta}{1}, \mathbf{v} \rangle = -\alpha, \; \mathbf{v}[1] > 0 \}$, and 
    \item $\pv{\mathbf{v}}{2} = [0 \;\; \kappa]^\top$, where $\alpha, \kappa > 0$.
\end{itemize}
See Figure \ref{fig:bad-example} for a visual depiction of such a setting.
Observe that a necessary condition for correctly intervening on units in $\pv{\cV}{0}$ is that the intervention policy should not assign intervention $d=2$ to any units with pre-treatment outcomes $\vy_{pre}$ such that $\|\vy_{pre} - \mathbf{v}\|_2 \leq \delta$, where $\mathbf{v} \in \pv{\cV}{0}$. An analogous statement holds for units in $\pv{\cV}{1}$. By~\Cref{def:ball}, any intervention policy which correctly intervenes on unit $\mathbf{v}$ if $\mathbf{v} \in \pv{\mathcal{V}}{0}$ or $\mathbf{v} \in \pv{\mathcal{V}}{1}$ must not assign intervention $d=2$ if $\Tilde{\vy}_{\mathbf{v},pre}$ is such that\looseness-1
\begin{equation*}
\begin{aligned}
    \langle \pv{\vbeta}{2} - \pv{\vbeta}{1}, \Tilde{\vy}_{\mathbf{v},pre} \rangle &\in [-\alpha - \delta \|\pv{\vbeta}{2} - \pv{\vbeta}{1}\|_2, -\alpha + \delta \|\pv{\vbeta}{2} - \pv{\vbeta}{1}\|_2]\\
    \text{or }
    \langle \pv{\vbeta}{2} - \pv{\vbeta}{0}, \Tilde{\vy}_{\mathbf{v},pre} \rangle &\in [-\alpha - \delta \|\pv{\vbeta}{2} - \pv{\vbeta}{0}\|_2, -\alpha + \delta \|\pv{\vbeta}{2} - \pv{\vbeta}{0}\|_2].\\
\end{aligned}
\end{equation*}

\noindent However if this condition is satisfied, it will be impossible to correctly intervene on unit $\mathbf{v}$ if $\mathbf{v} = \pv{\mathbf{v}}{2}$ and $(\kappa, \alpha)$ are small enough. To see this, note that in order for both 
\begin{equation*}
\begin{aligned}
    \langle \pv{\vbeta}{2} - \pv{\vbeta}{1}, \Tilde{\vy}_{\mathbf{v},pre} \rangle &> \delta \|\pv{\vbeta}{2} - \pv{\vbeta}{1}\|_2  -\alpha\\
    \text{and } \; \langle \pv{\vbeta}{2} - \pv{\vbeta}{0}, \Tilde{\vy}_{\mathbf{v},pre} \rangle &> \delta \|\pv{\vbeta}{2} - \pv{\vbeta}{0}\|_2 -\alpha\\
\end{aligned}
\end{equation*}
to hold,
\begin{equation*}
\begin{aligned}
\delta \|\pv{\vbeta}{2} - \pv{\vbeta}{1}\|_2 - \alpha &< (\pv{\vbeta}{2} - \pv{\vbeta}{1})[2](\kappa + \delta)\\
\text{and } \; \delta \|\pv{\vbeta}{2} - \pv{\vbeta}{0}\|_2 - \alpha &< (\pv{\vbeta}{2} - \pv{\vbeta}{0})[2](\kappa + \delta).
\end{aligned}
\end{equation*}
This implies that intervening perfectly on all units is not possible unless $\frac{1}{2} \kappa + \alpha > \delta(\sqrt{1.25} - 0.5)$, which does not hold for sufficiently small $\kappa$, $\alpha$.
\end{example}
